Just Go with the Flow: Self-Supervised Scene Flow Estimation

When interacting with highly dynamic environments, scene flow allows autonomous systems to reason about the non-rigid motion of multiple independent objects. This is of particular interest in the field of autonomous driving, in which many cars, people, bicycles, and other objects need to be accurately tracked. Current state-of-the-art methods require annotated scene flow data from autonomous driving scenes to train scene flow networks with supervised learning. As an alternative, we present a method of training scene flow that uses two self-supervised losses, based on nearest neighbors and cycle consistency. These self-supervised losses allow us to train our method on large unlabeled autonomous driving datasets; the resulting method matches current state-of-the-art supervised performance using no real world annotations and exceeds state-of-the-art performance when combining our self-supervised approach with supervised learning on a smaller labeled dataset.

==> Just Go with the Flow_ Self-Supervised Scene Flow Estimation/0-abstract.tex <==
\begin{abstract}
When interacting with highly dynamic environments, scene flow allows autonomous systems to reason about the non-rigid motion of multiple independent objects. This is of particular interest in the field of autonomous driving, in which many cars, people, bicycles, and other objects need to be accurately tracked. Current state-of-the-art methods require annotated scene flow data from autonomous driving scenes to train scene flow networks with supervised learning. As an alternative, we present a method of training scene flow that uses two self-supervised losses, based on nearest neighbors and cycle consistency.  These self-supervised losses allow us to train our method on large unlabeled autonomous driving datasets; the resulting method matches current state-of-the-art supervised performance using no real world annotations and exceeds state-of-the-art performance when combining our self-supervised approach with supervised learning on a smaller labeled dataset. 

%Our method .  

%loss provide equivalent supervisory signal to the ground truth flow error on the self-driving KITTI dataset as well as allow us to use unannotated datasets, such as nuScenes, to further improve generalization. 

%We show that a combination of nearest neighbor and cycle consistency loss provide equivalent supervisory signal to the ground truth flow error on the self-driving KITTI dataset as well as allow us to use unannotated datasets, such as nuScenes, to further improve generalization. 
\end{abstract}

==> Just Go with the Flow_ Self-Supervised Scene Flow Estimation/1-intro.tex <==
\section{Introduction}

For an autonomous vehicle, understanding the dynamics of the surrounding environment is critical to ensure safe planning and navigation. It is essential for a self-driving vehicle to be able to perceive the actions of various entities around it, such as other vehicles, pedestrians, and cyclists. In the context of data recorded as 3D point clouds, a motion can be estimated for each 3D point; this is known as scene flow, which refers to the 3D velocity of each 3D point in a scene. 
%It is the fundamental building block of motion for all semantic scene objects. 
%It describes the translation of each point in a scene. 
Its 2D analog, optical flow, is the projection of scene flow onto the image plane of a camera. An alternative to scene flow estimation is to use 3D object detection for object-level tracking and to assume that all points within a bounding box have the same rigid motion. However, in such a pipeline, errors in object detection can lead to errors in tracking. In contrast, scene flow methods can avoid such errors by directly estimating the motion of each 3D point.

% Previous methods for estimating scene flow often rely on optical flow and the 3D structure of the environment~\cite{herbst2013rgb, geometryvideo}; however, these methods do not make use of the depth information in estimating  the flow. 

%These networks learn a hierarchical feature representation over point clouds to predict the flow for each point. 

Recent state-of-the-art methods learn to estimate the scene flow from 3D point clouds~\cite{liu2019flownet3d,gu2019hplflownet,wang2018deep, pointpwcnet}. However, these methods are fully supervised and require annotated datasets for training.  Such annotations are costly to obtain as they require labeling the motion for every point in a scene. To compensate for the lack of real world data, learning-based methods for scene flow have been trained primarily on synthetic datasets and fine tuned on real world data. This requirement of labeled training data limits the effectiveness of such methods in real world settings.

\begin{figure}[t]
 	\centering
 	\includegraphics[trim={5 10 25 0}, clip,width=0.45\textwidth]{figures/overview_car.pdf}
 	\caption{We use two self-supervised losses to learn scene flow on large unlabeled datasets.  The ``nearest neighbor loss" penalizes the distance between the predicted point cloud (\textcolor{green}{green}) and each predicted point's nearest neighbor in the second point cloud (\textcolor{red}{red}).  To avoid degenerate solutions, we also estimate the flow between these predicted points (\textcolor{green}{green}) in the reverse direction back to the original point cloud (\textcolor{blue}{blue}) to form a cycle. The new predicted points from the cycle (\textcolor{magenta}{purple}) should align with the original points (\textcolor{blue}{blue}); the distance between these two set of points forms our second self-supervised loss: ``cycle consistency."}
 	\label{fig:cycle}
  	\vspace{-1em}
\end{figure} 

% 	The scene flow from point cloud $\matcal{X}$ to point cloud $\matcal{Y}$ and back produces a cycle that can be used to track points through time, from $\matcal{X}$ to $\matcal{\hat{X}}'$ to $\matcal{\hat{X}}$. The consistency of these loops acts as a supervisory signal to this flow}

%Scene flow also has advantages over rigid motion estimates, in that it does not require scene segmentation and can capture deformations in the objects and or their grouping. 

% Previous approaches to scene flow estimation have proposed solutions that assume certain structure over the point clouds. Either this structure is in the form of full rigid body motion of the point cloud or it involves constructing an occupancy grid over the space of point cloud in terms of voxels, lattice or graphs.

%Very recently, FlowNet3D suggested a method that assumes little-to-none structure prior over the point cloud.  This restricts their use on several large-scale real-world self-driving datasets where it is extremely hard to find per-point label for scene flow.




%limits their effectiveness in environments without such costly annotations. 

%The nearest neighbor loss operates by minimizing the euclidean distance between the predicted point and this pseudo-ground truth.

%\dave{This paragraph is too detailed - I will go back to shorten it later}
To overcome this limitation, we propose a self-supervised method for scene flow estimation. Using a combination of two self-supervised losses, we are able to mimic the supervision created by human annotation. Specifically, we use a cycle consistency loss, which  ensures that the scene flow produced is consistent in time (\ie we ensure that a temporal cycle ends where it started). We also use a nearest neighbor loss; due to the unavailability of scene flow annotations, we consider the nearest point to the predicted translated point, in the temporally next point cloud, as the pseudo-ground truth association.  Intuitively, the nearest neighbor loss pushes one point cloud to flow toward occupied regions of the next point cloud. We show that this combination of losses can be used to train a scene flow network over large-scale, unannotated datasets containing sequential point cloud data. An overview of our method can be found in Figure~\ref{fig:cycle}.

We test our self-supervised training approach using the neural network architecture of a state-of-the-art scene flow method~\cite{liu2019flownet3d}.  The self-supervision allows us to train this network on large-scale, unlabeled autonomous driving datasets. Our method matches the current state-of-the-art performance when no real world annotations are given. Moreover, our method exceeds the performance of state-of-the-art scene flow estimation methods when combined with supervised learning on a smaller labeled dataset. 

%temporal cycle consistency, approximation of the correspondences with nearest neighbor, and dataset augmentation

% \dave{This is a repeat of the previous paragraph}
% The key contributions of our paper are as follows. We introduce a novel self-supervised training method for learning scene flow estimation using self-supervised losses. We show that our self-supervised method can be applied to unannotated autonomous driving datasets to perform on-par with current state-of-the-art supervised approaches. We further show that our method is able to outperform state-of-the-art performance when combined with supervised learning on a smaller labeled dataset.

% We show that this self-supervision produces equivalent improvement to supervised training when used to fine tune scene flow estimators on real LIDAR scans of urban environments. Additionally, we show that using self-supervision in concert with the available supervised datasets produces superior results then supervision alone.  \dave{fix this}

%\textbf{re-write}
%We adapt the setting of the state-of-the-art method FlowNet3D where we directly deal with point clouds. Our method takes a pair of points clouds as input from two consecutive time frames and predicts the displacement vector for each point from first point cloud to the second point cloud. We take inspiration from point cloud registration methods as ICP and use the nearest neighbor of the point translated based on the predicted scene flow as its pseudo-ground truth label. We then iteratively optimize the predicted scene flow based on this pseudo-ground truth over time. Since the nearest neighbor can lead the prediction to a local optima, we further impose temporal cyclic consistency in the scene flow estimate. We do so by feeding the predicted point cloud as input to our model to predict the reverse scene flow which can map each translated point back to its original position.

%An autonomous vehicle is equipped with several sensors including LIDAR (LIght Detection And Ranging) to gather this necessary information about its environment. A LIDAR sensor captures a full 360 degrees scene information in the form of a sequence of point clouds comprising of hundreds of thousands of points per second. These point clouds serve as one of the most crucial source of data about the environment for the self-driving vehicle as it can be used for scene flow estimation as well as other tasks such as 3D classification and segmentation.

%Scene flow refers to the 3D translation of each point in the scene providing us the velocity vector associated with every single point. It is the fundamental building block of motion for all semantic scene objects. Estimating scene flow for tasks such as motion segmentation, visual odometry and SLAM has several advantages over other motion estimation methods. This is because scene flow does not assume any structural or motion prior making it more flexible to use. Moreover, since it is estimated directly in the 3D space, it circumvents the need of optic flow and disparity maps which are indirectly computed in 2D space by optimizing over RGB-D images. Scene flow estimation is particularly important for self-driving applications as point cloud data from LIDARs form the primary sensory information in this domain.

 

%We perform experiments on multiple point cloud datasets to demonstrate that these two techniques in combination allows to achieve performance comparable to supervised fine-tuning on the dataset.

==> Just Go with the Flow_ Self-Supervised Scene Flow Estimation/2-related.tex <==
\section{Related Work}
\paragraph*{Scene Flow} Vedula \etal~\cite{vedula1999three} first introduced the task of scene flow estimation. They propose a linear algorithm to compute it from optical flow. Other works involve joint optimization of camera extrinsics and depth estimates for stereo scene flow~\cite{valgaerts2010joint}, use of particle filters~\cite{hadfield2011kinecting}, local rigid motion priors~\cite{vogel20113d,vogel20153d,vogel2013piecewise, menze2015object}, and smoothness-based regularization~\cite{basha2013multi}. 

\vspace{-1em}
\paragraph*{Deep Scene Flow} 
State-of-the-art scene flow methods today use deep learning to improve performance.  
FlowNet3D~\cite{liu2019flownet3d} builds on PointNet++~\cite{qi2017pointnet++, qi2017pointnet} to estimate scene flow directly from a pair of point clouds.
Gu \etal ~\cite{gu2019hplflownet} produced similar results using a permutohedral lattice to encode the point cloud data in a sparse, structured manner.  The above approaches compute scene flow directly from 3D point clouds~\cite{liu2019flownet3d,gu2019hplflownet}. Methods involving voxelizations with object-centeric rigid body assumptions~\cite{Behl_2019_CVPR}, range images~\cite{vaquero2018deep}, and non-grid structured data~\cite{wang2018deep} have also been used for scene flow estimation. All of the above methods were trained either with synthetic data~\cite{mayer2016large} or with a small amount of annotated real-world data~\cite{kitti} (or both).  Our self-supervised losses enable training on large unlabeled datasets, leading to large improvements in performance.

%This algorithm was trained entirely with labeled data. The supervised training consists of synthetically annotated data with a small amount of hand annotated real data used for fine tuning. 

%Our approach is largely agnostic of the model used for scene flow estimation, since our method only relates to the loss used for training.

%Liu \etal~\cite{liu2019flownet3d} presented the first method, called FlowNet3D, which used deep learning for scene flow estimation by learning directly on point clouds. 








% FlowNet3D primarily comprises of three modules - point feature learning, point mixture, and flow refinement and three layers - set conv layer, flow embedding layer, and set upconv layer. It begins with hierarchically learning the point cloud features using its set conv layer inspired by PointNet++~\cite{qi2017pointnet++, qi2017pointnet}, in the first module. In the next module, the flow embedding layer takes as input two point clouds of consecutive time steps, $t$ and $t+1$, and learns the flow vector for each point in the first point cloud. Next, in the flow refinement module, the set-upconv layer up-samples the learned flow embeddings by propagating the point features of the downsampled points (source points) to the actual points (target points). Lastly, a linear regression layer is used to output the scene flow.

%FlowNet3D shows substantial improvement after fine tuning on the annotated real world data, showing benefits of using real data along with the synthetic dataset. 


\vspace{-1em}
\paragraph*{Self-Supervised Learning} Wang \etal ~\cite{wang2019learning} used self-supervised learning for 2D tracking on video. They propose a tracker which takes a patch of an image at time $t$ and the entire image at time $t-1$ to track the image patch in the previous frame. They define a self-supervised loss by tracking the patch forward and backward in time to form a cycle while penalizing the errors through cycle consistency and feature similarity. We take inspiration from this work for our self-supervised flow estimation on point clouds. Other works including self-supervisory signals are image frame ordering~\cite{misra2016shuffle}, feature similarity over time~\cite{wang2015unsupervised} for images, and clustering and reconstruction~\cite{hassani2019ICCV} from point clouds. While these can potentially be used for representation learning from 3D data, they cannot be directly used for scene flow estimation. Concurrent to our work, Wu \etal~\cite{pointpwcnet} showed that Chamfer distance, smoothness constraints, and Laplacian regularization can be used to train scene flow in a self-supervised manner.

%do not as directly map to scene flow as cycle consistency. 

% While tracking features on 2D images, the transformed features are normally a part of the next image frame. This ensures that real data can be used at each stage of the cycle and still maintain the correspondences between features. In 3D flow, the transformed points are rarely part of the next frame. In order to maintain correspondences through each transform, the transformed cloud needs to be used in the feature generation. This causes tracking error to both be integrated into the flow prediction and the featurization. 





==> Just Go with the Flow_ Self-Supervised Scene Flow Estimation/3-methods.tex <==
\section{Method}

\subsection{Problem Definition}
For the task of scene flow estimation, we have a temporal sequence of point clouds: point cloud $\mathcal{X}$ as the point cloud captured at time $t$ and point cloud $\mathcal{Y}$ captured at time $t+1$. There is no structure enforced on these point clouds and they can be recorded directly from a LIDAR sensor or estimated through a stereo algorithm. %No ordering is required, as our base algorithm, Flownet3D, is point order agnostic. 
Each point $p_i = \{x_i,f_i\}$ in point cloud $\mathcal{X}$ contains the Cartesian position of the point, $x_i \in \mathbb{R}^3$, as well as any additional information which the sensor produces, such as color, intensity, normals, etc, represented by $f_i \in \mathbb{R}^c$.

The scene flow, $\mathcal{D} = \{d_i\}^N, d_i \in \mathbb{R}^3$ between these two point clouds describes the movement of each point $x_i$ in point cloud $\mathcal{X}$ to its corresponding position $x_i'$ in the scene described by point cloud $\mathcal{Y}$, such that $x_i' = x_i + d_i$,  and $N$ is the size of point cloud $\mathcal{X}$. Scene flow is defined such that $x_i$ and $x'_i$ represent the same 3D point of an object moved in time. Unlike optical flow estimation, the exact 3D position of $x_i'$ may not necessarily coincide with a point in the point cloud $\mathcal{Y}$, due to the sparsity of the point cloud. Additionally, the sizes of $\mathcal{X}$ and $\mathcal{Y}$ may be different.


%Given two point clouds at consecutive time frames $\mathcal{X}$ and $\mathcal{Y}$, we define scene flow $\{d_i\}_N = \mathcal{D} \in \mathbb{R}^3$ as the displacement of a point $x$ in $\mathcal{X}$ to its corresponding position in the scene as described by point $p’$ in $P_{t+1}$. Therefore, 
%$$
%p’ = p + d
%$$
%Unlike optic flow, $p’$ is not necessarily part of $P_{t+1}$. Let $D_t$ describe the scene flow between $P_t$ and $P_{t+1}$ and comprise of the displacement of all points in $P_t$ to $P_{t+1}$. To estimate this scene flow $D_t$, we define a function $f: (P_{t}, P_{t+1}) \rightarrow D_t$ that learns a mapping between the two point clouds as input and gives the set of scene flow values $D_t$ as output. 

%\paragraph*{Tracking} Our method for self-supervised scene flow estimation uses the model of FlowNet3D as the tracking module to generate predictions for scene flow. During each iteration of training, we consider a pair of point clouds $P_t$ and $P_{t+1}$ at two consecutive time frames and feed a sample of $N$ points, $X \in P_t$ and $Y \in P_{t+1}$ from these two point clouds as input to the tracking module. The number of points $N$ in the sample depends on the capacity of the tracking module and theoretically can be equal to the total number of points in a given point cloud. The two samples $X$ and $Y$ need not have any pointwise correspondence between them and can be sampled differently from $P_t$ and $P_{t+1}$ at different training iterations. The tracking model processes the two point samples and predicts a scene flow vector, $V \in \mathbb{R}^{2048}$ corresponding to $P_1$. The value vi in V is the predicted displacement (scene flow) of point pi1 in P1 to a point $x_hat{i}$ in $P{t+1}$. Therefore,
%\begin{align}
%   \hat{x}_i &= x_i + v_i \quad \forall i \in \{1 \ldots N\} \\ 
%    \hat{X} &= X + V = \{\hat{x}_i \; | \; i = 1 \ldots N \}  
%\end{align}

%Even though this error directly encodes our flow accuracy, it

% of the transformed points $\hat{x}_i' = x_i + \hat{d}_i$ and $x_i' = x_i + d_i^*$
\vspace{-1em}
\paragraph*{Supervised Loss}
The true error associated with our task is the difference between the estimated flow $g(\mathcal{X}, \mathcal{Y}) = \mathcal{\hat{D}} = \{\hat{d}_i\}^N$ and the ground truth flow $\mathcal{D}^* = \{d^*_i\}^N$, 
\begin{align}
\mathcal{L}_{gt} = \frac{1}{N} \sum_i^N \|d_i^*-\hat{d}_i\|^2.   
\label{equ:gt}
\end{align}
The loss in Equation~\ref{equ:gt} is useful because it is mathematically equivalent to the end point error, which we use as our evaluation metric. However, computing this loss requires annotated ground truth flow $d^*_i$. This type of annotation is easy to calculate in synthetic data~\cite{mayer2016large}, but requires expensive human labeling for real world datasets. As such, only a small amount of annotated scene flow datasets are available ~\cite{menze2015joint, menze2018object}. While training on  purely synthetic data is possible, large improvements can often be obtained by training on real data from the domain of the target application.  For example, Lui \etal~\cite{liu2019flownet3d} showed an 18\% relative improvement after fine-tuning on a small amount of annotated real world data.  This result motivates our work to use self-supervised training to train on large unlabeled datasets. 

\begin{figure}[t]
 	\centering
 	\begin{subfigure}{0.23\textwidth}
 	\includegraphics[trim={70 250 70 250}, clip, width=\linewidth]{figures/car_loss_forward_30.pdf}
 	%\includegraphics[trim={20 230 20 200}, clip, width=\linewidth]{figures/car_loss_nn.pdf}
 	\caption{Nearest Neighbor Loss}
 	\end{subfigure}
 	%\vspace*{\fill}
  	\begin{subfigure}{0.23\textwidth}
 	\includegraphics[trim={70 250 70 250}, clip, width=\linewidth]{figures/car_loss_cycle_30.pdf}
 	\caption{Cycle Consistency Loss}
 	\end{subfigure}
 	\caption{Example of our self-supervised losses between consecutive point clouds $\mathcal{X}$ (\textcolor{blue}{blue}) and $\mathcal{Y}$ (\textcolor{red}{red}). We consider the point $x$ whose ground truth projected point $x'$ is not known during training time. $(a)$ Nearest Neighbor Loss is computed between the projected point $\hat{x}'$, predicted by the forward flow, and the closest point in $\mathcal{Y}$.  $(b)$ The Cycle Consistency Loss tracks this transformed point back onto its original frame, as point $\hat{x}''$, using the reverse flow, and computes the distance to its original position ${x}$.}
 	\label{fig:losses}
  	\vspace{-1em}
\end{figure} 

\vspace{-1em}
\paragraph*{Nearest Neighbor (NN) Loss}

%Unlike visual data such as images and videos, point clouds and their associated scene flow do not exhibit any structural prior. Therefore, the above mentioned optimization is under constrained and could lead to trivial solution. The above equation is still satisfied when $\hat{X}$ ends up being identical to $X$ with forward leg predicting zero displacement. So to discourage such scenario from happening, 

For large unlabeled datasets, since we do not have information about $d_i^*$, we cannot compute the loss in Equation~\ref{equ:gt}.  
In lieu of annotated data, we take inspiration from methods such as Iterative Closest Point~\cite{besl1992method} and use the nearest neighbor of our transformed point $\hat{x}_i' = x_i + \hat{d}_i$ as an approximation for the true correspondence. For each transformed point $\hat{x}_i' \in \hat{\mathcal{X}}'$, we find its nearest neighbor $y_j \in \mathcal{Y}$ and compute the Euclidean distance to that point, illustrated as $e_{NN}$ in Figure~\ref{fig:losses}a: 
\begin{equation}
    \mathcal{L}_{NN} = \frac{1}{N}\sum_i^N \min_{y_j \in \mathcal{Y}}\|\hat{x}_i' - y_j\|^2.
\label{equ:nn}
\end{equation}

Assuming that the initial flow estimate is sufficiently close to the correct flow estimate, this loss will bring the transformed point cloud and the target point cloud closer. This loss can, however, have a few drawbacks if imposed alone.  First, the true position of the point $x_i$ transformed by the ground truth flow, $x_i' = x_i + d_i^*$, may not be the same as the position of the nearest neighbor to $\hat{x}'$ (transformed by the \emph{estimated} flow) due to potentially large errors in the estimated flow, as illustrated in Figure~\ref{fig:losses}a.  Further, the position of $x_i'$ may not correspond with any point in $\mathcal{Y}$ if the point cloud $\mathcal{Y}$ is sufficiently sparse, as is common for point clouds collected by sparse 3D LIDAR for autonomous driving.  Finally, this loss does not penalize degenerate solutions where all of the points in $\mathcal{X}$ map to the same point in $\mathcal{Y}$; such a degenerate solution would obtain 0 loss under Equation~\ref{equ:nn}. To address these issues, we use an additional self-supervised loss: cycle consistency loss.

%which might lead to the collapse of the entire predicted point cloud to only a handful of points in point cloud $\mathcal{Y}$.  

%is minimized when each point in $\mathcal{X}$ is collocated with a point in $\mathcal{Y}$, which is not likely the optimal flow and can results in transformed points grouping to tightly around the points in the next cloud. %This behavior is countermanded by the cycle consistency loss, which is optimized when the flow function to be invariable, which is not the case if multiple points flow to the same point.

%Although the nearest neighbor for any given predicted point may not be its real correspondence, it is still a real point lying in $\mathcal{Y}$ which makes it a potential candidate for correspondence.

%Let $X^{nn}$ be the point sample comprising of all $x^{nn}_i$ corresponding to $\hat{x}_i$ for $i = 1, \ldots, N$. We then impose a euclidean distance based L2 regularization between $\hat{X}$ and $X^{nn}$, $\mathcal{L}_{nn}$ as follows,
%\begin{align}
%   \mathcal{L}_{nn} = || \hat{X} - X^{nn} ||_2 = \frac{1}{N} \sum_{i=1}^N \left( \hat{x}_i - %x^{nn}_i \right)^2 
%\end{align}
 %The $\mathcal{L}_nn$ loss pushes the predicted point away from $P_t$ and forces it to lie in the space of $P_{t+1}$. It therefore encourages the prediction to not collapse to a trivial solution. Moreover, even if the predicted point gets pushed over to an incorrect correspondence due to the above regularization, the cycle loss ensures that it does not affect the overall correspondence. Over the course of going through several diverse point samples while training, the cycle consistency neutralizes this side effect and preserves the correspondence between the point clouds.


%Cycle consistency is not sufficient as a supervisory signal, as this loss can be minimized by a flow of zero. To prevent this, we require the flow map each point in $\mathcal{X}$ to a region close to points in the second frame using a nearest neighbor loss. For each point $x' \in \mathcal{X}'$, we compute the nearest neighbor in $\mathcal{Y}$ and define this loss as:

%While optimizing the true loss, we are bringing the points in point cloud $\mathcal{X}$ closer to their corresponding location in the scene described by point cloud $\mathcal{Y}$, where this correspondence is defined by the true flow. We instead approximate this correspondence using the nearest neighbor of the transformed point, $\hat{x}$, resulting in a nearest neighbor loss of

 %While this will try to bring the two point clouds closer together, the independent nature of each of the flow vectors can lead to many points being attracted to a single point. To combat this we use a cycle loss similar to 

%The above constitutes the forward leg of our self-supervised approach. Unlike FlowNet3D, we assume that we do not have scene flow annotations during training. Therefore, we cannot simply optimize a supervised loss over the prediction $V$ from the tracking module. As part of our self-supervised method, we therefore propose a second flow prediction mechanism to encourage the model to learn just from the unannotated data. 

\vspace{-1em}
\paragraph*{Cycle Consistency Loss} 
To avoid the above issues, we incorporate an additional self-supervised loss: cycle consistency loss, illustrated in Figure~\ref{fig:losses}b. We first estimate the ``forward" flow as $\hat{\mathcal{D}} = g(\mathcal{X}, \mathcal{Y})$.  Applying the estimated flow $\hat{d}_i \in \hat{\mathcal{D}}$ to each point $x_i \in \mathcal{X}$ gives an estimate of the location of the point $x_i$ in the next frame: $\hat{x}_i' = x_i + \hat{d}_i$.  We then compute the scene flow in the reverse direction: for each transformed point $\hat{x}_i'$ we estimate the flow to transform the point back to the original frame, $\hat{\mathcal{D'}} = g(\mathcal{\hat{X}'}, \mathcal{X})$.  Transforming each point $\hat{x}_i'$ by this ``reverse" flow $\hat{d}_i'$ gives a new estimated point $\hat{x}_i''$.  If both the forward and reverse flow are accurate, this point $\hat{x}_i''$ should be the same as the original point $x_i$.  The error between these points, $e_{cycle}$, is the ``cycle consistency loss,"  given by
\begin{equation}
    \mathcal{L}_{cycle} = \sum_i^N \|\hat{x}_i'' - x_i\|^2.
\label{equ:cycle}
\end{equation}
A similar loss is used as a regularization in~\cite{liu2019flownet3d}.

% 

%We first use our estimated scene flow $\hat{d}_i$ to 

%$g(\hat{x}_i', x_i)$

%Let us define $\hat{\mathcal{X}}' = \mathcal{X} + \hat{\mathcal{D}}$ as the entire transformed point cloud.  We then 

% use the predicted flow $\hat{d}_i$ to track the point $x_i$ forward in time to the transformed point $x'$ in the temporal frame defined by $\mathcal{Y}$. This point is them tracked back to its original frame using $\hat{\mathcal{D}}' = \{\hat{d}_i'\}^N = g(\hat{\mathcal{X}}', \mathcal{X})$. Using the Euclidean distance between the transformed point and its original location we describe our cycle loss as: 

% \begin{equation}
%     \mathcal{L}_{cycle} = \sum \|g(\mathcal{X}, \mathcal{Y}) - g(\mathcal{X}', \mathcal{X}) \|^2,
% \end{equation}

% \noindent $d_{cycle}$ in Figure~\ref{fig:losses}. A similar loss is used as regularization in~\cite{liu2019flownet3d}.

%In order to maintain correspondences around the cycle, the transformed cloud $\hat{\mathcal{X}}'$ is used as an input in the reverse cycle $g(\mathcal{\hat{X}'}, \mathcal{X})$

However, we found that implementing the cycle loss in this way can produce unstable results if only self-supervised learning is used without any ground-truth annotations.  These instabilities appear to be caused by errors in the estimated flow which lead to structural distortions in the transformed point cloud $\hat{\mathcal{X}}'$, which is used as the input for computing the reverse flow $g(\mathcal{\hat{X}'}, \mathcal{X})$. This requires the network to simultaneously learn to correct any distortions in $\mathcal{\hat{X}'}$, while also learning to estimate the true reverse flow.
To solve this problem, we use the nearest neighbor $y_j$ of the transformed point $\hat{x}'_i$ as an anchoring point in the reverse pass.  Using the nearest neighbor $y_j$ stabilizes the structure of the transformed cloud while still maintaining the correspondence around the cycle. The effects of this stabilization are illustrated in Figure~\ref{fig:anchor}. As we are using the anchoring point as part of the reverse pass of the cycle, we refer to this loss as ``anchored cycle consistency loss''.

%compute both the inverse of the structural  distortions caused by errors in the forward pass and as well as the inverse of the true flow. 
% = \{\bar{d}_i'\}^N 
%, with respect to the original point cloud $\mathcal{X}$, and the convex combination of the transformed point and its nearest neighbor $\bar{\mathcal{X}} = \{\bar{x}_i'\}^N = \lambda \hat{x}_i' + (1-\lambda) y_j$. 

Specifically, we compute the anchored reverse flow as follows. First, we compute the forward flow as before, $\hat{\mathcal{D}} = g(\mathcal{X}, \mathcal{Y})$, which we use to compute the transformed point cloud $\hat{x}_i' = x_i + \hat{d}_i$.  We then compute anchor points $\bar{\mathcal{X}'} = \{\bar{x}_i'\}^N$ as a convex combination of the transformed point and its nearest neighbor $\bar{x}_i' = \lambda \hat{x}_i' + (1-\lambda) y_j$.  In our experiments, we find that $\lambda=0.5$ produces the most accurate results. Finally, we compute the reverse flow using these anchored points: $\bar{\mathcal{D}}' = g(\bar{\mathcal{X}}', \mathcal{X})$.  The cycle loss of Equation~\ref{equ:cycle} is then applied to this anchored reverse flow.  By using anchoring, some of the structural distortion of the predicted point cloud $\mathcal{\hat{X}'}$ will be removed in the anchored point cloud $\bar{\mathcal{X}'}$, leading to a more stable training input for the reverse flow.

Note that the cycle consistency loss also has a degenerate solution: the ``zero flow,", \ie $\hat{\mathcal{D}} = 0$, will produce 0 loss according to Equation~\ref{equ:cycle}.  However, the zero flow will produce produce a non-zero loss when anchored cycle consistency is used; thus anchoring helps to remove this degenerate solution.  Further, the nearest neighbor loss will also be non-zero for the degenerate solution of zero flow.  Thus, the local minima of each of the nearest neighbor and cycle consistency losses conflict, allowing their sum, $\mathcal{L} = \mathcal{L}_{NN} + \mathcal{L}_{cycle}$, to act as a stable surrogate for the true error.

%If we instead look at our problem as learning a continuous flow field over 3D space that we query at points defined by our point clouds, we can use two structurally stable point clouds for both the forward and reverse flow estimates. We are now learning a function $d = f(x |\mathcal{X},\mathcal{Y})$ and the reverse flow can be described as $d' = f(x' | \mathcal{X},\mathcal{Y})$, as opposed to $d' = f(x' | \mathcal{X},\mathcal{X}')$ where $\mathcal{X}'$ may contain substantially structural deformations, example shown in Figure 

\begin{figure}[t]
 	\centering
 	\begin{subfigure}{0.23\textwidth}
 	\includegraphics[trim={20 70 20 70}, clip, width=\linewidth]{figures/car_noise.png}
 	\caption{}
 	\end{subfigure}
 	\hspace*{\fill}
  	\begin{subfigure}{0.23\textwidth}
 	\includegraphics[trim={20 70 20 70}, clip, width=\linewidth]{figures/car_anchor.png}
 	\caption{}
 	\end{subfigure}
 	\caption{Compounding errors cause problems in estimating reverse flow using the transformed point cloud. $(a)$ Large flow prediction errors degrade the structure of the transformed cloud $\hat{\mathcal{X}}'$ (shown in \textcolor{green}{green}). Thus, computing the reverse flow between $\hat{\mathcal{X}}'$ (\textcolor{green}{green}) and $\mathcal{X}$ (\textcolor{blue}{blue}) is an ill-posed task.
 	$(b)$ Using the nearest neighbor points (\textcolor{red}{red}) as anchors, we are able to stabilize the transformed cloud $\bar{\mathcal{X}}'$ (\textcolor{cyan}{cyan}), thus retaining important structural information.}
 	\label{fig:anchor}
  	\vspace{-1em}
\end{figure}


%We take the displaced point sample, $\hat{X}$  as predicted by the forward leg of our approach and feed it as input along with $X$ into the tracking module. The tracking module again processes these two point samples and predicts a backward scene flow vector, $V’ \in \mathbb{R}^{2048}$ corresponding to $\hat{X}$. Each value $v’{i} \in V’$ is now the predicted displacement (scene flow) of point $\hat{x}_i \in \hat{X}$ to a point $\hat{x}’ \in P_t$. Therefore,
%\begin{align*}
%    \hat{x}_i' &= \hat{x}_i + v'_i \quad \forall i \in \{1 \ldots N\} \\ 
%    \hat{X}' &= \hat{X} + V' = \{\hat{x}_i' \; | \; i = 1 \ldots N \}  
%\end{align*}
%This constitutes the backward leg of our self-supervised approach, thus completing the flow prediction cycle. Since the forward and backward scene flow are essentially the displacement of a given point in forward and reverse direction, the point $\hat{x}_i’ \in P_t$ at the end of the backward leg should be the same point as $x_i$ at the beginning of the forward leg. Therefore,
%\begin{align}
%    x_i &= \hat{x}_i’ \quad \forall i \in \{1 \ldots N\}
%\end{align} 
%We enforce this relationship by imposing a euclidean distance based cycle loss, $\mathcal{L}_{cycle}$ as part of the objective function. 
%\begin{align}
%    \mathcal{L}_{cycle} = || X - \hat{X}' ||_2 = \frac{1}{N} \sum_{i=1}^N \left( x_i - \hat{x}_i' \right)^2
%\end{align}
%This enables us to circumvent the need for scene flow annotations at the end of the forward leg and make use of the cycle consistency of scene flow to learn from the data in a self-supervised fashion.

%\paragraph*{Loss}
%The objective function $\mathcal{L}$ of our method comprises of the above mentioned loss functons, $\mathcal{L}_{cycle}$ and $\mathcal{L}_{nn}$, and is given as follows,

%\begin{equation}
%    \mathcal{L} = \mathcal{L}_{cycle} + \mathcal{L}_{nn}
%\end{equation}

 
%During inference, we remove the backward flow prediction mechanism and treat the output of the forward prediction mechanism as the predicted scene flow between $P_t$ and $P_{t+1}$.


%We design a model that estimates the 3D scene flow between the points of the consecutive point clouds. The goal is to estimate the scene flow in a self-supervised manner by tracking a point of the point cloud forward and then backwards in time while reducing the cycle and Nearest Neighbor loss. For our model, the input would be a set of two point clouds from consecutive time frames, point cloud 1 being X = \{ (xi, fi) | i = 1 to n \} and point cloud 2 being Y = \{ (yj, fj)| j = 1 to n \} where xi, yj E R3 are xyz coordinates of a single point in a scene and fi, fj are the features of a point e.g: color features, Lidar intensity. Since NuScenes dataset did not have the color features, we try to extract the colors from the images. The detailed explanation of the color extraction is in section ..... While working on the point cloud, we focus on both the XYZ coordinates and the feature space F of a point.

%For a given point P in the point cloud 1, our tracker T takes as input both the point clouds at time t and time t+1, and tries to find the position of this point in the point cloud 2. Our tracker is based on the framework on Flownet3d which estimates the scene flow for every point in the point clouds of the first frame. Since we do not have the correspondences between the points of the two point clouds, once the tracker finds the location of the point P in the point cloud 2 as Q, we apply 1-nearest neighbor. The 1-NN takes as input point Q and the whole point cloud 2 to find out the nearest neighbor of this point, R. We treat this nearest neighbor as the corresponding point for point P. Moreover, the result of 1-NN can also be treated as a pseudo ground truth. Since, it is possible that the nearest neighbor is not the actual corresponding point, we impose a 1-NN loss over the point Q and the point R. The 1-NN loss is the Euclidean distance between the 1-NN point and the point predicted in the point cloud at time t. While minimizing this loss, our model is able to learn the right correspondences with time. 

%After the forward cycle, we re-apply our tracker for the backward cycle where the inputs would be the point Q and the point cloud 1. Our tracker finds the location point Q in the point cloud 1, S. We impose a cycle loss over the predicted point, S and the original point P. 

%\begin{figure}[t]
% 	\centering
% 	\includegraphics[width=0.5\textwidth]{figures/skip_interpolation.png}
% 	\caption{}
% 	\label{fig:flow_field}
%\end{figure}

%\section{Implementation}
%\subsection{Flownet3D}
%Our method for self-supervised scene flow estimation builds upon the state-of-the-art method for supervised scene flow estimation FlowNet3D~\cite{liu2019flownet3d}. FlowNet3D is an end-to-end network which estimates the scene flow between two point clouds in a supervised manner. Primarily, it has three modules - point feature learning, point mixture, and flow refinement and three layers - set conv layer, flow embedding layer, and set upconv layer. It begins with hierarchically learning the point cloud features using its set conv layer, PointNet++, in the first module. This layer takes as input a single point cloud and down-samples it into n regions using farthest point sampling and extracts local features of each region using a multi-layer perceptron.  In the next module, the flow embedding layer takes as input two point clouds of consecutive time steps, t and t+1 and learns the flow vector for each point in the first point cloud. Following this, in the module of flow refinement, the set-upconv layer up-samples the learned flow embeddings by propagating the point features of the downsampled points (source points) to the actual points (target points). Lastly, a linear regression layer is used to output the scene flow.

%\subsection{Self-supervised scene flow estimation}
%Figure {} illustrates the network architecture of our self-supervised scene flow prediction model.
\vspace{-1em}
\paragraph*{Temporal Flip Augmentation}
% During self-supervised training, we augment the training set by flipping the order of consecutive point clouds. We find that, if we do not do this, there is a forward motion bias in the data which sometimes leads the network to predict a flow equal to the average forward speed of the training set. This temporal flip augmentation results in the removal of this bias, since the network now sees an equal number of frames in which the point cloud appears to be moving in the ``forward" as well as the ``reverse" directions. 

%
Having a dataset of point cloud sequences in only one direction may generate a motion bias which may lead to the network predicting the flow equal to the average forward speed of the training set. To reduce this bias, we augment the training set by flipping the point clouds, i.e, reversing the flow. With this augmentation, the network sees an equal number of point cloud sequences having a forward motion and a backward motion. 
%

%Because the supervisory signal is based purely on the point clouds being in close proximity in time, this can be done without modifying any of the data. 


==> Just Go with the Flow_ Self-Supervised Scene Flow Estimation/4-experiments.tex <==
\section{Experiments}

We run several experiments to validate our self-supervised method for scene flow estimation for various levels of supervision and different amounts of data. First, we show that our method, with self-supervised training on large unlabeled datasets, can perform as well as supervised training on the existing labeled data.
Next, we investigate how our results can be improved by combining self-supervised learning with a small amount of supervised learning, exceeding the performance of purely supervised learning. Finally, we explore the utility of each element of our method through an ablation study.

% we consider a scenario in which no training annotations are available; thus we compare our self-supervised approach with a baseline which only trains on synthetic data~\cite{liu2019flownet3d}. 


%can generalize to the real world unannotated data by exploring both pure self-supervision as well as augmented supervised training. 

\subsection{Implementation Details}
For all data configurations (our method and the baseline), we initialize our network with the parameters of the Flownet3D model~\cite{liu2019flownet3d} pre-trained on the FlyingThing3D dataset~\cite{mayer2016large}. We compare our self-supervised training procedure to a baseline which uses supervised fine-tuning on the KITTI dataset~\cite{kitti}.  The baseline used in the comparison is the same as in Liu \etal~\cite{liu2019flownet3d}, except that we increase the number of training iterations from 150 epochs (as described in the original paper) to 10k epochs in order to keep the number of training iterations consistent with that used in our self-supervised method. We see that this change leads to a small improvement in the baseline performance, which we include in the results table. %At each iteration, a batch of 8 scenes are selected and a random pair of consecutive point clouds are sampled.

%For the baseline, supervised training on the KITTI dataset, 

\begin{figure*}[t]
 	\centering
 	\includegraphics[trim={0 0 0 50}, clip, width=\textwidth]{figures/self-supervised-unsupervised-f3d.pdf}
 	\caption{Scene flow estimation between point clouds at time $t$ (\textcolor{red}{red}) and $t+1$ (\textcolor{green}{green}) from the KITTI dataset trained without any labeled LIDAR data. Predictions from our self-supervised method, trained on nuScenes and fine-tuned on KITTI using self-supervised learning is shown in \textcolor{blue}{blue}; the baseline with only synthetic training is shown in \textcolor{magenta}{purple}. In the absence of real-world supervised training, our method clearly outperforms the baseline method, which overestimate the flow in many regions. (Best viewed in color)}
 	\label{fig:qual_no_ground_truth}
\end{figure*}


\begin{figure*}[t]
 	\centering
 	%\includegraphics[width=\textwidth]{figures/nuscenes_comparison.pdf}
 	\begin{subfigure}{0.48\textwidth}
 	\includegraphics[trim={0 0 900 50}, clip, width=\textwidth]{figures/nuscenes_comparison.pdf}
 	\caption{Ours (Self-Supervised Fine Tuning)}
 	\end{subfigure}
 	%\vspace*{\fill}
  	\begin{subfigure}{0.48\textwidth}
 	\includegraphics[trim={920 0 0 50}, clip, width=\textwidth]{figures/nuscenes_comparison.pdf}
 	\caption{Baseline (No Fine Tuning)}
 	\end{subfigure}
 	\caption{Comparison of our self-supervised method to a baseline trained only on synthetic data, shown on the nuScenes dataset. Scene flow is computed  between point clouds at time $t$~(\textcolor{red}{red}) and $t+1$~(\textcolor{green}{green}); the point cloud that is transformed using the estimated flow is in shown in \textcolor{blue}{blue}. In our method, the predicted point cloud has a much better overlap with the point cloud of the next timestamp (\textcolor{green}{green})  compared to the baseline. Since nuScenes dataset does not provide any scene flow annotation, the supervised approaches cannot be fined tuned to this environment.}
 	\label{fig:qual_nuscenes}
 	\vspace{-1em}
\end{figure*}


\begin{figure*}[ht!]
 	\centering
 	\includegraphics[trim={0 0 0 40}, clip, width=\textwidth]{figures/supervised_new.pdf}
 	\caption{Scene flow estimation on LIDAR data from the KITTI dataset between point clouds at time $t$ (\textcolor{red}{red}) and $t+1$ (\textcolor{green}{green}). Our method, which is trained on nuScenes using self-supervised learning and then fine-tuned on KITTI using supervised learning, is shown in \textcolor{blue}{blue}. The baseline method is fine-tuned only on KITTI using supervised training and is shown in \textcolor{magenta}{purple}. While in aggregate, both methods well estimate the scene flow, adding self-supervised training on nuScenes (\textcolor{blue}{blue}) enables our predictions to more closely match the next frame point cloud (\textcolor{green}{green}). In several  scenes, the purely supervised method (\textcolor{magenta}{purple}) underestimates the flow, staying too close to the initial point cloud (\textcolor{red}{red}). (Best viewed in color)}
 	\label{fig:qual_supervised}
 	%\vspace{-1em}
\end{figure*}


\subsection{Datasets}

\paragraph*{KITTI Vision Benchmark Suite}  KITTI~\cite{kitti} is a real-world self-driving dataset. There are 150 scenes of LIDAR data in KITTI collected using seven scans of a Velodyne 64 LIDAR, augmented using 3D models, and annotated with ground truth scene flow~\cite{menze2018object}. For our experiments under both self-supervised and supervised settings, we consider 100 out of 150 scenes for training and the remaining 50 scenes for testing. Ground points are removed from every scene using the pre-processing that was performed in previous work~ \cite{liu2019flownet3d}. Every scene consists of a pair of point clouds recorded at two different times as well as the ground truth scene flow for every point of the first point cloud. 

\vspace{-1em}
\paragraph*{nuScenes} The nuScenes~\cite{nuscenes2019} dataset is a large-scale public dataset for autonomous driving. It consists of 850 publicly available driving scenes in total from Boston and Singapore. The LIDAR data was collected using a Velodyne 32 LIDAR rotating at 20 Hz. This is in contrast to the 64-beam Velodyne rotating at 10 Hz used for the KITTI dataset.  This difference in sensors leads to a difference in data sparsity that creates a distribution shift between KITTI and nuScenes.  This distribution shift necessitates additional training on KITTI beyond our self-supervised training on nuScenes.  Nonetheless, our results show a substantial benefit from the self-supervised training on nuScenes.

Since the nuScenes dataset~\cite{nuscenes2019} does not contain scene flow annotations, we must use self-supervised methods when working with this dataset. In our experiments, out of the 850 scenes available, we use 700 as the train set and the rest 150 as the validation set. Similar to KITTI, we remove the ground points from each point cloud using a manually tuned height threshold.

\begin{table*}[h]
\centering
\begin{tabular} {l|c c c}
\toprule
 Training Method & EPE (m) $\downarrow$ & ACC (0.05) $\uparrow$ & ACC (0.1) $\uparrow$ \\
\hline
\hline
No Fine Tuning & 0.122 & 25.37\% & 57.85\% \\
KITTI (Supervised) & 
0.100 & 31.42\% & 66.12\% \\
\hline
Ablation: KITTI (Self-Supervised)  & 0.126 & 32.00\% & 73.64\% \\
Ours: nuScenes (Self-Supervised) + KITTI (Self-Supervised)  & 0.105 & 46.48\% & 79.42\% \\
Ours: nuScenes (Self-Supervised) + KITTI (Supervised) & \textbf{0.091} & \textbf{47.92\%} & \textbf{79.63\%} \\
\bottomrule
\end{tabular}
%}
\caption{Comparison of levels of supervision on KITTI dataset. The nearest neighbor + anchored cycle loss is used for nuScenes (self-supervised) and KITTI (self-supervised). All methods are pretrained on FlyingThings3D\cite{mayer2016large} and ground points are removed for KITTI and nuScenes datasets.}\label{tbl:supervision}
\vspace{-1em}
\end{table*}

\subsection{Results}
We use three standard metrics to quantitatively evaluate the predicted scene flow when the ground truth annotations of scene flow are available. Our primary evaluation metric is End Point Error (EPE) which describes the mean Euclidean distance between the predicted and ground truth transformed points, described by Equation~\ref{equ:gt}. We also compute accuracy at two threshold levels, Acc(0.05) as the percentage of scene flow prediction with an EPE~$<~0.05$m or relative error~$<5\%$ and Acc(0.1) as percentage of points having an EPE~$<0.1$m or relative error~$<~10\%$, as was done for evaluation in previous work~\cite{liu2019flownet3d}. 

%These thresholds match the standard accuracy threshold computed in scene flow research.

%\vspace{-1em}
\subsubsection{Quantitative Results}

% While self-supervision is able improve on the network trained on synthetic dataset, more data may be needed to generalize using this indirect training signal. Unlike previous works, we are not restricted to annotated point cloud datasets. Our method can be used on any sequentially collected point cloud dataset. There have been several point cloud datasets published containing real LIDAR captures taken in urban scenes, but most of them do not contain scene flow annotations. While, these datasets could not be used for supervised scene flow learning, using a unsupervised loss allows us access to this data. 

% Adding the nuScenes dataset to our training set gives us almost 5x the real world data, adding 5.5 hrs to the 1.4 hrs of data available in KITTI. 

\paragraph*{Self-supervised training:}
Unlike previous work, we are not restricted to annotated point cloud datasets; our method can be trained on any sequential point cloud dataset. There are many point cloud datasets containing real LIDAR captures of urban scenes, but most of them do not contain scene flow annotations. Due to lack of annotations, these datasets can not be utilized for supervised scene flow learning. In contrast, our self-supervised loss allows us to easily integrate them into our training set. The combination of these datasets (KITTI + NuScenes) contains 5x more real data than using KITTI alone.
%\vspace{-1em}

%first consider the case in which we train our method without any

%\paragraph*{Setup}  
The results are shown in Table~\ref{tbl:supervision}.
To show the value of self-supervised training, we evaluate the performance of our method without using any  ground-truth annotations.  We first pre-train on the synthetic FlyingThings3D dataset; we then perform self-supervised fine-tuning on the large nuScenes dataset followed by further self-supervised fine-tuning on the smaller KITTI dataset (4th row: ``Ours: nuScenes (Self-Supervised) + KITTI (Self-Supervised)").  As can be seen, 
using no real-world annotations, we are able to achieve an EPE of 0.105~m.  This outperforms the baseline of only training on synthetic data (``No Fine Tuning").  Even more impressively, our approach performs similarly to the baseline which 
pre-trains on synthetic data and then 
does supervised fine-tuning  on the KITTI dataset (``KITTI (Supervised)"); our method has a similar EPE and outperforms this baseline in terms of accuracy, despite not having access to any annotated training data. This result shows that our method for self-supervised training, with a large enough unlabeled dataset, can match the performance of supervised training.

%the benefit of self-supervised training, which can be performed on large unlabeled datasets even when no real world training annotations are available.


% no annotations are available for training. We compare this to the baseline model which trains only on the synthetic FlyingThings3D dataset with no fine-tuning (``No Fine Tuning"). The ideal baseline is in fact matching supervised performance, so we also compare to the model pretrained on FlyingThings3D with supervised fine-tuning on the KITTI dataset (``KITTI (Supervised)"). For our method, we similarly pre-train on the FlyingThings3D dataset; we then fine-tune the model using self-supervised training on the large NuScenes dataset, followed by further self-supervised fine-tuning on the smaller KITTI dataset (``Ours: nuScenes (Self-Supervised) + KITTI (Self-Supervised)").

% We begin with training our self-supervised model on the nuScenes dataset using the combination of Nearest Neighbor Loss and Anchored Cycle loss. Since we wish to use Flownet3D as our scene flow estimation module, we initialize our network with Flownet3D weights pretrained on FlyingThing3D dataset~\cite{mayer2016large,liu2019flownet3d}. Once the model has been trained on nuScenes, we fine-tune on KITTI in a self-supervised manner. For the comparison with the baseline, we use the Flownet3D model pretrained on FlyingThings3D without any fine-tuning on KITTI.
%\vspace{-1em}

%\paragraph*{Quantitative Study} 
% The results are shown in Table~\ref{tbl:supervision}. As can be seen, 
% using only unannotated data, we are able to achieve an EPE of 0.1053 m, which is much better than the baseline of training only on synthetic data (``No Fine Tuning").  

% This result shows the benefit of real-world self-supervised fine-tuning, which can be performed even when no real world training annotations are available.

% We can also compare our method to a baseline which assumes access to the labeled KITTI dataset for supervised training (2nd row).  Compared to this baseline, our self-supervised method achieves a similar EPE and much better accuracies, despite not having access to any annotated training data.
% This result shows the benefit of pre-training on an large unlabeled dataset (NuScenes). 

\vspace{-1em}
\paragraph*{Self-supervised + Supervised:} Finally, we show the value of combining our self-supervised learning method with a small amount of supervised learning. For this analysis, we perform self-supervised training on NuScenes as above, followed by supervised training on the much smaller KITTI dataset.  The results are shown in the last row of Table~\ref{tbl:supervision}.

As can be seen, this approach of self-supervised training followed by supervised fine-tuning outperforms all other methods on this benchmark, obtaining an EPE of 0.091, outperforming the previous state-of-the-art result which used only supervised training.  This shows the benefit of self-supervised training on large unlabeled datasets to improve scene flow accuracy, even when scene flow annotations are available.

While Table~\ref{tbl:supervision} only shows results using the FlowNet3D~\cite{liu2019flownet3d} architecture, we note that our method also outperforms the results of HPLFlownet~\cite{gu2019hplflownet}~(EPE of 0.1169) and all models they compare against as well.
%\vspace{-1em}

% \paragraph*{Setup} To evaluate our method on the real-world datasets having ground truth flow annotations, we fine tune our model on KITTI. For our method, we pretrain the model on nuScences using our self-supervised loss, and then introduce the KITTI data for supervised fine tuning. For the baseline, we use Flownet3d which is supervised fine tuned over the KITTI dataset. Both models are initialized with Flownet3D weights pretrained on FlyingThings3D. 

% \paragraph*{Quantitative Results} By first training on the large amount of unannotated data available in nuScenes using the  combination  of  Nearest Neighbor Loss and Anchored Cycle Loss and then fine tuning on KITTI using the supervised loss, we are able to outperform the state-of-the-art on KITTI, obtaining an EPE of 0.0912. This is due to the fact that the additional self-supervised data allowed the model to generalize better to new real world scenes. While we only report the results of FlowNet3D~\cite{liu2019flownet3d} in Table \ref{tbl:supervision}, our method also outperforms the results of HPLFlownet~\cite{gu2019hplflownet}~(EPE of 0.1169) and all models they compare against.
% %\vspace{-1em}

% nearly the same performance as supervised fine tuning, in terms of endpoint error, by producing an error estimate of only 8 mm greater that those given by the supervised model. Additionally, we achieve a significantly higher accuracy with respect to both standard error thresholds. We compare our self-supervised method to the supervised fine tuning describe in~\cite{liu2019flownet3d}, over various levels of supervision and self-supervision, using the same initial weights across all methods. 

%No Fine Tuning represents the model trained only on the FlyingThings3D dataset~\cite{mayer2016large}. 

Figure \ref{fig:epe_vs_mag} provides an analysis on the correlation between average endpoint error and the magnitude of the ground truth flow.  As can be seen, our method consistently outperforms the baseline at almost all flow magnitudes. 

%We performed a similar analysis, with respect to local point density, computed using a 0.1m radius ball around each point, and found no correlation between EPE and point density.

\begin{figure}[t]
 	\centering
 	\includegraphics[width=0.47\textwidth]{figures/self-super-vs-unsuper-new.png}
 	\caption{Analysis of average EPE (m) with respect to ground truth flow magnitudes (m). Flow estimates are binned by ground truth flow magnitude and a confidence interval of 95\% is shown for all results.}
 	\label{fig:epe_vs_mag}
 	\vspace{-1em}
\end{figure} 

%In this figure, both our method and the baseline have not seen the ground truth. 

%\vspace{-1em}
\subsubsection{Qualitative Analysis}
\paragraph*{Self-supervised training - KITTI results:} 
Next we perform a qualitative analysis to visualize the performance of our method.
We compare our method (synthetic pre-training + self-supervised training on nuScenes + self-supervised training on KITTI) compared to the baseline of synthetic training only.  Results on KITTI are shown in Figure~\ref{fig:qual_no_ground_truth}. The figure shows the point clouds captured at time $t$ and $t+1$  in red and green, respectively. The predictions from our method are shown in blue and the baseline predictions are shown in purple. As shown, our scene flow predictions (blue)  have a large overlap with the point cloud at time $t+1$ (green). On the other hand, the baseline predictions (purple) do not overlap with the point cloud at time $t+1$.  The baseline, trained only on synthetic data, fails to generalize to the real-world KITTI dataset. On the contrary, our self-supervised approach can be fine tuned on any real world environment and shows a significant improvement over the baseline. 

%The scene flow prediction from our method coincides well with the point cloud $\mathcal{Y}$ across scene objects showing wide range of motion. 

%We can observe from the figure that the translated points predicted by the baseline are considerably farther from the point cloud $\mathcal{Y}$, in comparison to the predictions of our method, and the difference is more pronounced for scene objects exhibiting large motion. We believe that 

\vspace{-1em}
\paragraph*{Self-supervised training - nuScenes results:}
%\subsubsection{Self-supervised results on nuScenes}

% \begin{table*}[]
% \centering
% \begin{tabular}{l|c}
% \toprule
% Method & Mean Nearest Neighbor Distance \\ 
% \hline
% Baseline (No fine tuning) & \\
% Self-Supervised (Nearest Neighbor) & \\
% Self-Supervised (NN + Anchored Cycle) & \\ 
% \bottomrule
% \end{tabular}
% \caption{Mean Nearest Nearest Neighbor Distance on nuScenes dataset. Self-Supervised methods are trained on the nuScences dataset. All methods are pretrained on FlyingThings3D using supervisory training.}
% \end{table*}

%\paragraph*{Qualitative Study} 

Next, we visualize the performance of our method on the nuScenes dataset.  Note that, because nuScenes does not have scene flow annotations, only qualitative results can be shown on this dataset. For this analysis, our method is pre-trained on synthetic data (FlyingThings3D) as before and then fine-tuned on nuScenes in a self-supervised manner. No scene flow annotations for nuScenes are available, so we compare to a baseline which is trained only on synthetic data.  

The results on nuScenes are shown in Figure~\ref{fig:qual_nuscenes}. These results again showcase the advantages of self-supervision on real world data over purely synthetic supervised training. As before, the figure shows the point clouds captured at time $t$ and $t+1$ in red and green respectively. The predictions are shown in blue, with our method on the left (Fig.~\ref{fig:qual_nuscenes}a) and the baseline on the right (Fig.~\ref{fig:qual_nuscenes}b).  As shown, our scene flow predictions (left figure, blue) have a large overlap with the point cloud at time $t+1$ (green). On the other hand, the baseline predictions (right figure, blue) do not overlap with the point cloud at time $t+1$. 

%from our method are shown in blue and the baseline predictions are shown in purple. As shown, our scene flow predictions (blue)  have a large overlap with the point cloud at time $t+1$ (green). On the other hand, the baseline predictions (purple) do not overlap with the point cloud at time $t+1$. 

% In each scene, point cloud $\mathcal{X}$ is shown in red and point cloud $\mathcal{Y}$ is shown in green. The translated points predicted by our model and the baseline are shown in blue and purple respectively. As we can observe in the figure, the prediction from our self-supervised model has a much better overlap with point cloud $\mathcal{Y}$ as compared to the prediction from the baseline method. 

The low performance of the baseline can again be attributed to its training on synthetic data and its inability to generalize to real-world data.  For the nuScenes data, no scene flow annotations exist, so only self-supervised learning is feasible to improve performance.

% where the scale of scene flow values is considerably different than the real-world nuScenes dataset. Due to this discrepancy in the magnitude of scene flow between the datasets, the baseline is unable to generalize well to nuScenes. Moreover, since nuScenes does not have ground truth scene flow, the purely supervised baseline cannot be fine tuned to improve its prediction on this environment. Since our method does not rely on ground truth scene flow labels, it can be easily applied to such datasets to obtain a considerably better scene flow prediction. 



\begin{table}[]
\centering
\footnotesize
\setlength\tabcolsep{2pt}
\begin{tabular}{c|c|c|c||c|c|c}
\toprule
\multicolumn{7}{l}{Self-Supervised Training (nuScenes + KITTI)} \\ \midrule
NN Loss & Cycle Loss & Anchor Pts & Flip & EPE (m) & ACC (0.05) & ACC (0.1) \\ 
\hline
\checkmark & \checkmark & \checkmark & \checkmark & 0.105 & 46.48\% & 79.42\% \\ 
\checkmark & \checkmark & \checkmark &  & 0.107 & 40.03\% & 72.20\% \\
\checkmark & \checkmark &  &  & 0.146 & 30.21\% & 48.57\% \\
\checkmark &  &  &  & 0.108 & 42.00\% & 78.51\% \\
 &  &  &  & 0.122 & 25.37\% & 57.85\% \\
\hline \hline
\multicolumn{7}{l}{Self-Supervised (nuScenes) + Supervised Training (KITTI)} \\ \hline
NN Loss & Cycle Loss & Anchor Pts & Flip & EPE (m) & ACC (0.05) & ACC (0.1) \\ 
\hline
\checkmark & \checkmark & \checkmark & \checkmark & {0.091} & {47.92\%} & {79.63\%} \\ 
\checkmark & \checkmark & \checkmark &  & {0.093} & {40.69\%} & {74.50\%} \\
\checkmark & \checkmark &  &  & 0.092 & 30.76\% & 72.94\% \\
\checkmark &  &  &  & 0.114 & 31.24\% & 64.58\% \\
 &  &  &  & 0.100 & 31.42\% & 66.12\%\\ \bottomrule
\end{tabular}
\caption{Ablation analysis: We study the effect of the different self-supervised losses and data augmentation. Top: Models use self-supervised training on nuScenes and KITTI; Bottom: Models use self-supervised training on nuScenes followed by supervised training on KITTI.}\label{tbl:ablation}
\vspace{-1em}
\end{table}

%All models are trained using the self-supervised losses on nuScenes. Fine-tunning on KITTI is trained using self-supervised losses (top) and supervised loss (bottom)

% study on the KITTI dataset

\begin{table}
\centering
\footnotesize
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c | c | c | c}
\toprule
$\lambda$ & EPE (m)$\downarrow$ & ACC (0.05)$\uparrow$ & ACC (0.1)$\uparrow$ \\ 
\hline
0   & 0.120 & 24.09\% & 73.20\% \\
0.25 & 0.122 &  26.41\% & 65.57\% \\
0.5 & \textbf{0.105} & \textbf{46.48\%} & \textbf{79.42\%} \\
0.75 &  0.125 & 23.59\% & 62.96\% \\
1   & 0.149 & 22.97\% & 49.58\% \\
\bottomrule
\end{tabular}
\caption{Effect of varying the $\lambda$ parameter for ``anchoring" the Cycle Consistency Loss. Results are shown for self-supervised training on nuScenes + KITTI.}\label{tbl:cycle_lambda}
\vspace{-1em}
\end{table}

%\subsubsection{Supervised fine tuning on KITTI}
%\paragraph*{Setup} 

\vspace{-1em}
\paragraph*{Self-supervised + supervised training - KITTI results:} 
Finally, we show the value of combining our self-supervised learning method with a small amount of supervised learning, compared to only performing supervised learning.  For our method, we perform synthetic pre-training, followed by self-supervised fine-tuning on nuScenes, followed by supervised fine-tuning on the much smaller KITTI dataset. We compare to a baseline which only performs synthetic pre-training followed by supervised fine-tuning KITTI.



% To evaluate our method on the real-world datasets having ground truth flow annotations, we fine tune our model on KITTI. For our method, we pretrain the model on nuScences using our self-supervised loss, and then introduce the KITTI data for supervised fine tuning. For the baseline, we use Flownet3d which is supervised fine tuned over the KITTI dataset. Both models are initialized with Flownet3D weights pretrained on FlyingThings3D. 

% \paragraph*{Quantitative Results} By first training on the large amount of unannotated data available in nuScenes using the  combination  of  Nearest Neighbor Loss and Anchored Cycle Loss and then fine tuning on KITTI using the supervised loss, we are able to outperform the state-of-the-art on KITTI, obtaining an EPE of 0.0912. This is due to the fact that the additional self-supervised data allowed the model to generalize better to new real world scenes. While we only report the results of FlowNet3D~\cite{liu2019flownet3d} in Table \ref{tbl:supervision}, our method also outperforms the results of HPLFlownet~\cite{gu2019hplflownet}~(EPE of 0.1169) and all models they compare against.
%\vspace{-1em}

%\paragraph*{Qualitative Study} 

Qualitative results can be seen in Figure~\ref{fig:qual_supervised}. The figure shows the point clouds captured at time $t$ and $t+1$  in red and green, respectively. The predictions from our method are shown in blue and the baseline predictions are shown in purple. As shown, our scene flow predictions (blue)  have a large overlap with the point cloud at time $t+1$ (green), whereas the baseline predictions (purple) do not. 

% In each scene, point cloud $\mathcal{X}$ is shown in red and point cloud $\mathcal{Y}$ is shown in green. The translated points predicted by our method and the baseline are shown in blue and purple respectively. As we can observe in the figure, the prediction from our self-supervised method has a much closer overlap with point cloud $\mathcal{Y}$ as compared to the prediction from the baseline.

The baseline predicts a small motion, keeping the transformed cloud (purple) too close to the initial position (red). As discussed above, this bias towards small motion is likely due to the training of the baseline over a synthetic dataset, which affects the generalization of the baseline to real-world datasets where objects exhibit different types of motion than seen in simulation. By training over a significantly larger unlabeled dataset, our method is able to avoid overfitting and generalizes better to the scenes and flow patterns which were not present in the synthetic dataset.

\begin{figure}[t]
 	\centering
 	\includegraphics[trim={0 0 0 100}, clip, width=\columnwidth]{figures/cycle_vs_forward_comparison.pdf}
 	\caption{Ablation study comparing our self-supervised method with both nearest neighbor loss and anchored cycle consistency loss (\textcolor{blue}{blue}) compared to training only using the nearest neighbor loss (\textcolor{magenta}{purple}). Scene flow is computed between point clouds from the KITTI dataset at time $t$ (\textcolor{red}{red}) and $t+1$ (\textcolor{green}{green})}
 	\label{fig:nuscenes_ablation}
  	\vspace{-1em}
\end{figure}

\subsubsection{Ablation Studies}
%We perform some experiments as part of the ablation studies: (1). Augment the data with the flipped/reversed point clouds, (2). Change the input to the model for backward flow prediction. 

%The advantage of implementing the anchored cycle consistency loss can be seen best in the augmented supervised results, as well as

We test the importance of each component of our method by running a series of ablation studies. Table~\ref{tbl:ablation} shows the effect of iteratively removing portions of our method in both the purely self-supervised (top) and self-supervised + supervised (bottom) training.
The benefits of anchored cycle consistency loss (compared to only using nearest neighbor loss) can be seen in  Table~\ref{tbl:ablation} (bottom) as well as in Figure~\ref{fig:nuscenes_ablation}. 

The benefits of anchoring is apparent by the large drop in performance for self-supervised training (top) when anchoring is removed.  
 Introducing the anchor point cloud as part of the backward flow greatly improves performance when only self-supervised training is used (Figure~\ref{fig:nuscenes_ablation}, top).
  This suggests that having anchored point clouds stabilizes the training of the cycle consistency loss. Additionally, we evaluate the sensitivity of our system to the selection of the anchoring parameter, $\lambda$. Table~\ref{tbl:cycle_lambda} shows that we obtain the best results with $\lambda=0.5$, \ie using the average of the predicted and nearest points. Overall, these analyses show the benefits of each component of our method. Further ablation analysis can be found in the supplement.
 
 %We further observe that by introducing the temporal flip augmentation in the train set, the model sees a wider variety of scene flow directions which reduces any directional bias present in self-driving datasets.




==> Just Go with the Flow_ Self-Supervised Scene Flow Estimation/5-conclusion.tex <==
%\vspace{-1em}
\section{Conclusion}

% In this paper, we proposed a self-supervised method for training scene flow algorithms using a combination of cycle consistency in time and nearest neighbor losses. We validated this method on the widely used KITTI self-driving dataset and show that our self-supervision method produces equivalent results when compared to direct supervision, opening the door to fine tuning on arbitrary environments and online flow learning using only sequential point clouds. Further, we show that augmenting existing annotated datasets with unannotated data using our self-supervised approach out performs the existing baselines on the KITTI scene flow datasets. 

In this work, we propose a self-supervised method for training scene flow algorithms using a combination of cycle consistency in time and nearest neighbor losses. Our purely self-supervised method is able to achieve a performance comparable to that of the supervised methods on the widely used KITTI self-driving dataset. We further show that when supervised training is augmented with self-supervision on a large-scale, unannotated dataset, the results exceed the current state-of-the-art performance. Our self-supervision method opens the door to fine-tuning on arbitrary datasets that lack scene flow annotations. 

%and future investigation into online flow learning using only sequential point clouds. 


\subsection*{Acknowledgements}
This work was supported by the CMU Argo AI Center for Autonomous Vehicle Research and a NASA Space Technology Research Fellowship.
